Transfer Once, Ask Locally: Compact Audio-Visual Memory for On-Device Question Answering

Audio-visual question answering on lightweight user devices requires balancing speed, memory usage, privacy, and communication. One approach is to run audio-visual encoders on a server and a lightweight language decoder on the user device, keeping questions local while offloading media encoding. However, transferring and processing the full multimodal representation remains costly. We propose a training-free, query-agnostic token pruning framework that constructs a compact, reusable memory before transmission. We define video spatio-temporal blocks and aligned audio windows as players and estimate their importance through Monte Carlo Shapley valuation. We use an embedding coverage objective that combines query-independent utility with cross-modal redundancy calibration and rewards unimodal diversity through marginal coverage gains. We retain the original token embeddings of high-scoring players under a limited token budget and transfer the resulting memory once for reuse across subsequent local questions. Experiments on Video-MME, Daily-Omni, and Video-Holmes using video-SALMONN 2+ (3B) and video-SALMONN 2 Pro (4B) show that our method achieves the best or tied-best QA accuracy among the compared compression methods across all evaluated settings. On Daily-Omni with video-SALMONN 2+ (3B) at 80\% pruning, our method improves accuracy by 12.86--14.62 percentage points over these methods while achieving the lowest device-side LLM prefill and decoding latency, with up to $1.92\times$ decoding speedup at comparable embedding memory usage.

==> sec/0_abstract.tex <==
\begin{abstract}
\textcolor{blue}{Divya: Remove the term personalized, personalized would mean we use user details to answer questions, which we do not do here} Personalized audio-visual question answering on \textcolor{blue}{Divya: user devices requires balancing speed, memory, privacy and communication}lightweight devices requires balancing privacy, computation, and communication.
\textcolor{blue}{Divya: Is this how prior worjk does it? If so, state it, else say something like, one approach to alleviating this issue is ... }Running audio-visual encoders on a server and a lightweight language decoder on the user device keeps questions local, but transferring the full multimodal representation remains costly.
We propose a training-free, query-agnostic token pruning framework that constructs a compact, reusable memory before transmission.
\textcolor{blue}{Divya: Use active voice, we define video spat... as players ... and compute...}Video spatio-temporal blocks and aligned audio windows are treated as players, whose importance is estimated through Monte Carlo Shapley valuation.
An embedding coverage objective combines query-independent utility with cross-modal redundancy calibration and encourages unimodal diversity through marginal coverage gains.\textcolor{blue}{Divya: again, active voice, its good to have the voice consistent throughout the paragraph}
% This design accounts for the possibility that similar audio and visual content provides duplicated evidence rather than additional information.
We retain the original token embeddings of high-scoring groups under a restricted token budget.
The resulting memory is transferred once and reused for subsequent local questions, reducing communication and multimodal context processing while keeping user queries on the device.
Experiments on standard video question-answering benchmarks show that our method achieves higher QA accuracy than all compared token compression methods.\textcolor{blue}{Divya: Add some numbers here, on x benchmarks, y models, a-b percent improvement}
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Personalized media services play an important role in everyday life, as different users seek explanations and information tailored to their interests and needs. \textcolor{blue}{Divya: Persoanlized would mean using user data, which dont use here, answers are to generic questions, so avoid the term personalzied; I would focus more on the lightweight part to directly bridge the narrative to token pruning}
Second-screen companion applications address these needs by extending the viewing experience from a shared display (i.e. server side) to lightweight personal devices that provide content-related information based on viewers' interests~\cite{10.1145/3025453.3025459}.
Recent work on accessible video interfaces illustrates the value of customized descriptions and conversational question answering for blind and low-vision viewers~\cite{cheema2026vidscribe}.
Answering questions locally on personal devices can help protect user privacy by keeping questions and responses on the device. \textcolor{blue}{Divya: Good point to keep, doing it on device helps privacy}
For example, Apple's Foundation Models framework supports local language processing without sending user data to a server~\cite{apple2025foundationframework}.

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{fig/fig1.pdf}
  \caption{
  A server processes video and audio into a compact memory and transfers it once to a personal device.
  The device reuses this memory to answer multiple questions locally, keeping user queries on the device.
  To construct the compact memory, we propose a novel token selection method. 
  Fig.~\ref{fig:overview} provides an overview of our framework and the proposed method.}
  \label{fig:teaser}
\end{figure}

Multimodal foundation models~\cite{videollava, videollama, videosalmonn2} offer a natural way to answer viewers' questions about audio-visual content.
However, deploying this capability involves a trade-off between privacy and device resources.
On the one hand, processing everything on a server requires transmitting users’ questions and potentially personal context beyond their devices, raising privacy concerns and incurring additional communication overhead through repeated exchanges of questions and responses.
On the other hand, running the entire model locally instead places substantial computational and memory demands on lightweight devices, particularly for long-form video and audio.
We therefore consider a collaborative deployment (see Fig.~\ref{fig:teaser}): a server or playback host runs the audio-visual encoders, while each user's device runs a lightweight language decoder and handles questions locally.\textcolor{blue}{Divya: Why? Has prior work done this? Is this the most pragmatic way?}
Such a division requires considering communication alongside computation~\cite{10.1145/3093337.3037698}.
Even with the encoders offloaded, long-form content can produce a large number of multimodal tokens.
Transferring these tokens consumes bandwidth, while storing and processing them increases device memory usage and inference latency.
The central challenge is therefore to reduce the transferred representation while preserving the evidence needed to answer users' questions.

Pruning visual and audio tokens before they enter the device-side LLM offers a way to reduce both communication and local inference costs.
However, several existing approaches rely on information unavailable during server-side memory construction.
Query-guided methods such as PruneVid~\cite{prunevid} require the user's question, whereas our setting keeps questions and personal context on the device.
Pruning inside the device-side LLM, as in FastV~\cite{fastv}, leaves the initial token transfer unchanged and still requires processing the input through the layers preceding pruning.
These approaches therefore cannot directly construct a query-agnostic memory for one-time transfer and reuse across future questions.
Pre-LLM compression methods provide applicable building blocks, but selecting complementary audio-visual evidence remains a key challenge.
OmniZip~\cite{omnizip} uses audio retention to guide video token allocation and cross-modal similarity to consolidate audio anchors.
However, high cross-modal similarity may also indicate duplicated evidence.
When audio and video convey the same information, retaining both may consume budget without adding much coverage.
Whether prioritizing such shared evidence best preserves information for unknown questions therefore remains an open question.

To address these challenges, we propose a training-free, query-agnostic framework that constructs a compact audio-visual memory before transmission to the user device.
We organize video tokens into spatio-temporal blocks and audio tokens into aligned temporal windows, treating each group as a player.
Rather than scoring players in isolation, we evaluate their average marginal contributions to an embedding coverage objective through Monte Carlo Shapley estimation.
The objective combines embedding-based utility with cross-modal redundancy calibration, while encouraging unimodal diversity through coverage.
This formulation assigns less additional credit to already represented content and downweights evidence duplicated across modalities.
% We allocate the shared token budget between modalities using query-independent utility scores and retain players according to their estimated Shapley values.
The selected groups preserve their original token embeddings, forming a reusable memory that is transferred once.
A lightweight on-device decoder then answers subsequent questions using this memory, reducing communication and local processing costs while keeping user questions on the device.

Our contributions are threefold:
\begin{itemize}
  \item We formulate audio-visual token pruning as query-agnostic memory construction at the server--device interface.
  The compact memory supports one-time transfer and repeated local question answering while keeping user queries on the device.

  \item We develop a training-free framework that treats structured audio-visual token groups as players and estimates their marginal contributions through Monte Carlo Shapley valuation.
  Its embedding coverage objective combines modality-specific utility and cross-modal redundancy calibration, encouraging unimodal diversity and complementary evidence under a restricted token budget.

  \item We evaluate our framework on standard video question-answering benchmarks, including video-SALMONN 2+ (3B).
  Our method outperforms all compared token compression methods in QA accuracy. \textcolor{blue}{Divya: Add numbers, a-b percent improvement, what benchmarks? list all models - qwen, videosalmon }
\end{itemize}

